End-to-End Modeling Hierarchical Time Series Using Autoregressive Transformer and Conditional Normalizing Flow based Reconciliation

Multivariate time series forecasting with hierarchical structure is pervasive in real-world applications, demanding not only predicting each level of the hierarchy, but also reconciling all forecasts to ensure coherency, i.e., the forecasts should satisfy the hierarchical aggregation constraints. Moreover, the disparities of statistical characteristics between levels can be huge, worsened by non-Gaussian distributions and non-linear correlations. To this extent, we propose a novel end-to-end hierarchical time series forecasting model, based on conditioned normalizing flow-based autoregressive transformer reconciliation, to represent complex data distribution while simultaneously reconciling the forecasts to ensure coherency. Unlike other state-of-the-art methods, we achieve the forecasting and reconciliation simultaneously without requiring any explicit post-processing step. In addition, by harnessing the power of deep model, we do not rely on any assumption such as unbiased estimates or Gaussian distribution. Our evaluation experiments are conducted on four real-world hierarchical datasets from different industrial domains (three public ones and a dataset from the application servers of Alipay's data center) and the preliminary results demonstrate efficacy of our proposed method.

==> application.tex <==
Our method is successfully deployed on application servers of our company, the world's leading company of payment technology, to forecast server traffic.  Our company has a giant cluster of application servers to support its complex financial Internet business, separated into numerous \textit{Internet Data centers} (IDC), which is a facility where an organization or a service provider rely on as computation infrastructure.  In order to improve the efficiency of resource utilization, pre-scheduling application services is essential, for which we need to predict the traffic to facilitate resource management decisions.  In Company's IDCs, the deployment of application services adopts a hierarchical structure.  Specifically, each deployment consists of three levels: the upper layer is call \textit{app deployment unit}, and the bottom deployment unit is called \textit{zone}, which is divided into Gzone, Rzone, and Czone. Each zone is then divided into multiple groups, as shown in Figure 8 below.
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth,,height=0.6\linewidth]{fig/figure-10.jpg}
  \caption{A deployment example of Company's application service}
\end{figure}
In practice, the hierarchical prediction for the service traffic at each deployment level facilitates the precise management and scheduling \cite{qiu2020firm}. In the experiments above as shown in Table 1, we perform $T+8h$ predictions on the data collected from real-world servers in our company over the past 90 days to verify the effectiveness of our method. The prediction of server traffic can be used not only for efficient resource management/allocation in IDCs, but also for achieving \textbf{energy savings} and \textbf{reducing carbon dioxide emissions} through server scheduling management \cite{qiu2020firm} to promote \textbf{carbon neutrality}. Our method was deployed before the Double 11 shopping festival and according to the certification of \textit{China Environmental United Certification Center} (CEC), a reduction of \textbf{394 tons of carbon dioxide} and a saving of \textbf{640,000 kWh of electricity} were achieved during the shopping festival, marking a critical step for our company's goal towards \textit{carbon neutrality} by 2030.  Our forecasting algorithm has been running robustly and contiuously since then, contributing to the energy efficiency of Company's cloud service.
